The Age, Stellar Content and Star Formation Timescale of the B59 Dense Core

We have used moderate resolution, near-infrared spectra from the SpeX spectrograph on the NASA Infrared Telescope facility to characterize the stellar content of Barnard 59 (B59), the most active star-forming core in the Pipe Nebula. Measuring luminosity and temperature sensitive features in the spectra of 20 candidate YSOs, we identified likely background giant stars and measured each star's spectral type, extinction, and NIR continuum excess. We find that B59 is composed of late type (K4-M6) low-mass (0.9--0.1 M_sun) YSOs whose median stellar age is comparable to, if not slightly older than, that of YSOs within the Rho Oph, Taurus, and Chameleon star forming regions. Deriving absolute age estimates from pre-main sequence models computed by D'Antona et al., and accounting only for statistical uncertainties, we measure B59's median stellar age to be 2.6+/-0.8 Myrs. Including potential systematic effects increases the error budget for B59's median (DM98) stellar age to 2.6+4.1/-2.6 Myrs. We also find that the relative age orderings implied by pre-main sequence evolutionary tracks depend on the range of stellar masses sampled, as model isochrones possess significantly different mass dependencies. The maximum likelihood median stellar age we measure for B59, and the region's observed gas properties, suggest that the B59 dense core has been stable against global collapse for roughly 6 dynamical timescales, and is actively forming stars with a star formation efficiency per dynamical time of ~6%. This maximum likelihood value agrees well with recent star formation simulations that incorporate various forms of support against collapse, such as sub-critical magnetic fields, outflows, and radiative feedback from protostellar heating. [abridged]

==> arxiv/t1.tex <==
\begin{deluxetable*}{lcccccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablecaption{IRTF/SpeX SXD Observing Log for Candidate B59 Members \label{tab:obslog_B59}}
\tablehead{
  \colhead{Source} &
  \colhead{} &
  \colhead{} &
  \colhead{2MASS} &
  \colhead{2MASS} &
  \colhead{2MASS} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{NTT} &
  \colhead{NTT}\\
  \colhead{ID} &
  \colhead{RA} &
  \colhead{Dec} &
  \colhead{$J$} &
  \colhead{$H$} &
  \colhead{$K_{s}$} &
  \colhead{itime} &
  \colhead{slit} &
  \colhead{J S/N} &
  \colhead{H S/N} &
  \colhead{K S/N} &
  \colhead{$H$} &
  \colhead{$K$} }\startdata
\textrm{[BHB2007]} 1 &  17:11:03.93 & -27:22:55.08 &  10.46 &   8.99 &   7.76 &   240 &     0.3 &  152/52 &   243/49 &  293/114 & 9.29 & 8.29\\
\textrm{[BHB2007]} 2 &  17:11:04.12 & -27:22:59.44 &   9.75 &   8.79 &   8.05 &   240 &     0.3 &  136/48 &   155/35 &   151/73 & 8.91 & 8.56\\
\textrm{[BHB2007]} 3 &  17:11:11.83 & -27:26:54.98 &  14.09 &  12.62 &  11.76 &  6240 & 0.5/0.3 &   58/13 &   108/26 &   186/40 & 12.69& 11.77\\
\textrm{[BHB2007]} 4 &  17:11:14.46 & -27:26:54.45 &  11.62 &  10.42 &   9.63 &  1920 &     0.3 &  277/41 &   344/48 &   347/57 & 10.62& 9.77 \\
\textrm{[BHB2007]} 5 &  17:11:16.26 & -27:20:28.82 &  11.23 &   9.70 &   9.07 &  1440 &     0.3 &  132/57 &   168/23 &   158/56 & 9.70& 9.08 \\
\textrm{[BHB2007]} 6 &  17:11:16.31 & -27:25:14.50 &  10.58 &   9.37 &   8.75 &   960 &     0.3 &  203/40 &   234/41 &   227/63 & 9.37& 8.75 \\
\textrm{[BHB2007]} 7 &  17:11:17.28 & -27:25:08.16 &  13.61 &  10.82 &   8.77 &  1920 &     0.3 &  58/12  &   261/34 &   325/92 & 10.58& 8.77 \\
\textrm{[BHB2007]} 8 NW & 17:11:18.24&-27:25:48.94 &\nodata & \nodata & \nodata &  1920 &     0.3 & \nodata &      2/0 &    59/17 & 16.01& 12.87 \\
\textrm{[BHB2007]} 8 SE & 17:11:18.32&-27:25:49.53 & $>$18.4 & 15.12 & 11.95  &  1920 &     0.3 & \nodata &      3/0 &    60/16 & 15.35& 12.78 \\
\textrm{[BHB2007]} 9 &  17:11:21.55 & -27:27:41.70 &  12.74 &  10.57 &   8.98 &  2400 &     0.3 &  122/31 &   230/42 &   348/69 & 11.215&8.98  \\
\textrm{[BHB2007]} 12 & 17:11:25.08 & -27:24:42.67 &  16.52 &  13.61 &  11.57 &  2880 &     0.5 &  15/3   &   63/13  &    154/34 & 13.32&11.58  \\
\textrm{[BHB2007]} 13 NW&17:11:26.95 &-27:23:48.40 &  11.88 &  10.14 &   9.08 & 1440  &     0.3 &   84/32 &   126/42 &   120/3  & 10.14&9.08 \\
\textrm{[BHB2007]} 14 & 17:11:27.28 & -27:25:28.32 &  13.17 &  10.65 &  9.11  &  2400 &     0.5 &  120/21 &   351/31 &  494/111 & 10.57& 11.44 \\
\textrm{[BHB2007]} 15 & 17:11:29.43 & -27:25:36.89 &  13.28 &  11.74 &  10.70 &  2400 &     0.5 &  149/24 &   291/30 &   359/46 & 11.74&10.58  \\
\textrm{[BHB2007]} 16 & 17:11:30.35 & -27:26:28.91 &  11.91 &  10.00 &   8.89 &  1680 &     0.3 &   49/19 &    64/32 &    64/66 & 10.23&9.19  \\
\textrm{[BHB2007]} 17 & 17:11:41.00 & -27:18:36.82 &  10.64 &   8.75 &   7.54 &   960 &     0.3 &  146/18 &    150/8 &   106/19 & 8.75&7.54  \\
\textrm{[BHB2007]} 18 NE&17:11:41.73& -27:25:50.26 & \nodata& \nodata & \nodata &  480  &     0.3 &  216/37 &   287/39 &   312/50 & 10.46&9.86  \\
\textrm{[BHB2007]} 18 SW &  \nodata &      \nodata & \nodata& \nodata& \nodata&  1440 &     0.3 &   72/32 &    76/40 &    69/55 & \nodata& \nodata \\
\textrm{[BHB2007]} 19 & 17:11:43.17 & -27:30:58.54 &  14.09 &  12.75 &  11.91 &  1920 &     0.3 &   47/11 &    92/17 &   127/26 & 12.66&11.74  \\
\textrm{[BHB2007]} 20 & 17:12:00.20 & -27:20:18.10 &  10.54 &   9.64 &   9.17 &   960 &     0.3 &  119/51 &   116/51 &   146/81 & 9.641& 9.17\\
\tableline
V359 Oph & 17:08:54.28 & -27:12:33.03 & 9.73 & 9.12 & 8.80 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  \nodata \\
LkH$\alpha$ 345 & 17:10:48.04 & -27:40:51.19 & 9.60 & 8.69 & 8.35 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  \nodata \\
KK Oph A & 17:10:08.07 & -27:15:18.24 & 9.07 & 7.23 & 5.80 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  \nodata
\enddata
\end{deluxetable*}


==> arxiv/t2.tex <==
\begin{deluxetable*}{lcccccccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablecaption{IRTF/SpeX SXD Observing Log for Pipe/TW Hya Sources \label{tab:obslog_Pipe_TWHya}}
\tablehead{
  \colhead{Source} &
  \colhead{} &
  \colhead{} &
  \colhead{2MASS} &
  \colhead{2MASS} &
  \colhead{2MASS} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{SXD} &
  \colhead{SXD}\\
  \colhead{ID} &
  \colhead{RA} &
  \colhead{Dec} &
  \colhead{$J$} &
  \colhead{$H$} &
  \colhead{$K_{s}$} &
  \colhead{itime} &
  \colhead{slit} &
  \colhead{J S/N} &
  \colhead{H S/N} &
  \colhead{K S/N}}
\startdata
\textrm{[CLR2010]} 1  &17:14:51.08 & -27:22:39.96 &  10.26 &   8.89 &   8.16 &  360 & 0.3 &   447/55 &   654/54 &   498/84 \\
\textrm{[CLR2010]} 2 NE &  \nodata &      \nodata &\nodata & \nodata&\nodata &  480 & 0.3 &   100/44 &   107/33 &   106/36 \\
\textrm{[CLR2010]} 2 SW &17:14:56.49&-27:31:08.08 &  10.42 &   9.56 &   9.04 &  480 & 0.3 &    86/32 &   100/32 &   108/35 \\
\textrm{[CLR2010]} 3 & 17:15:59.37 & -27:00:24.75 &   6.99 &   5.72 &   5.13 &  120 & 0.3 &  507/116 &   794/19 &   935/58 \\
\textrm{[CLR2010]} 4 & 17:19:06.05 & -27:06:18.95 &  13.07 &   9.69 &   7.50 &  360 & 0.3 &     25/5 &    136/9 &   141/38 \\
\textrm{[CLR2010]} 5 & 17:20:12.47 & -26:55:09.40 &   9.12 &   7.58 &   6.67 &  720 & 0.3 &   229/30 &   241/10 &   294/24 \\
\textrm{[CLR2010]} 6 & 17:22:31.01 & -23:53:48.76 &   7.52 &   6.06 &   5.13 &  120 & 0.3 &   357/17 &    474/9 &   884/21 \\
\textrm{[CLR2010]} 7 & 17:26:15.14 & -26:44:37.31 &   9.16 &   7.13 &   5.79 &  240 & 0.3 &   180/64 &   180/20 &   182/62 \\
\textrm{[CLR2010]} 8 & 17:27:41.56 &  -26:53:46.7 &  10.12 &   7.87 &   6.19 &  240 & 0.3 &    38/15 &   146/43 &   488/49 \\
\textrm{[CLR2010]} 9 & 17:29:54.08 & -25:59:12.79 &   7.29 &   5.83 &   5.05 &  120 & 0.3 &   423/78 &   726/18 &   971/56 \\
\tableline 				   	    	      	 			    		
        TW Hya 12 &   11:21:05.6 &    -38:45:16   &   9.00 &   8.33 &   8.05 &  480 & 0.3 &  343/113 &   392/46 &   346/88 \\
     CD 29-8887 A &   11:09:14.0 &    -30:01:39   &   7.85 & \nodata&   7.18 &  360 & 0.3 &  628/110 &   776/50 &  717/100 \\
     CD 29-8887 B &   11:09:14.2 &    -30:01:38   &   9.09 &\nodata &   7.99 &  480 & 0.3 &  434/107 &   451/51 &  352/103 \\
     CD 33-7795 A &   11:31:55.4 &    -34:36:27   &   7.67 &   6.99 &   6.74 &  360 & 0.3 &  574/105 &   674/55 &   608/93 \\
     CD 34-7390 A &   11:21:17.3 &    -34:46:47   &   8.43 &   7.73 &   7.49 &  120 & 0.3 &   241/96 &   290/48 &   267/91 \\
     CD 34-7390 B &   11:21:17.5 &    -34:46:44   &\nodata &\nodata &\nodata &  240 & 0.3 &  376/116 &   473/46 &   430/87 \\
     CD 36-7429 A &   11:48:24.2 &    -37:28:49   &   8.60 &   7.95 &   7.68 &  480 & 0.3 &   392/99 &   420/47 &   343/87 \\
     CD 36-7429 B &   11:48:24.0 &    -37:28:49   &  10.06 &   9.41 &   9.14 &  480 & 0.3 &  219/115 &   265/51 &   238/86 \\
  GSC 6659-1080 A &   11:32:41.3 &    -26:51:55   &   8.34 &   7.66 &   7.43 &  120 & 0.3 &  239/104 &   285/48 &   262/81 \\
  GSC 6659-1080 B &   11:32:41.2 &    -26:52:08   &   9.84 &   9.28 &   9.01 &  240 & 0.3 &   181/77 &   202/44 &   201/49 \\
    GSC 7766-074 &   12:35:04.4 &    -41:36:39    &   9.12 &   8.48 &   8.19 &  360 & 0.3 &   227/99 &   258/51 &   224/87 \\
           GY 17 &   16:26:23.7 &  -24:43:13.9    &   9.39 &   8.40 &   7.85 &  480 & 0.3 &   371/71 &   435/57 &   377/93 \\
          GY 250 &   16:27:19.5 &  -24:41:40.5    &   9.42 &   8.63 &   8.41 &  480 & 0.3 &   540/93 &   619/48 &   514/91 \\
          GY 292 &   16:27:33.1 &  -24:41:15.7    &  11.32 &   9.13 &   7.81 &  480 & 0.3 &   136/29 &   151/41 &   114/85 \\
           GY 93 &  16:26:41.26 &    -24:40:18    &  10.77 &   9.77 &   9.27 &  480 & 0.3 &   303/55 &   330/39 &   281/42 \\
       HD 98800 A &   11:22:05.5 &  -24:46:39.7   &   6.40 &   5.76 &   5.59 &  360 & 0.3 &   863/84 &   970/46 &   783/77 \\
       Hen 3600 A &   11:10:28.0 &    -37:31:53   &   8.22 &   7.60 &   7.28 &  360 & 0.3 &  269/117 &   325/49 &   315/68 \\
       Hen 3600 B &  11:10:28.05 &  -37:31:54.2   &   8.63 &   8.07 &   7.80 &  360 & 0.3 &   213/95 &   245/49 &   223/75 \\
    SSS 1207-324 &   12:07:27.4 &    -32:47:00    &   8.62 &   8.02 &   7.75 &  360 & 0.3 &  319/112 &   364/53 &   329/78 \\
          TW Hya &   11:01:52.0 &    -34:42:17    &   8.22 &   7.56 &   7.30 &  480 & 0.3 &  501/110 &   640/57 &  615/117 \\
   TYC 7760-0283 &   12:15:30.8 &    -39:48:42    &   8.17 &   7.50 &   7.31 &  360 & 0.3 &  434/111 &   525/46 &   461/82 
\enddata
\end{deluxetable*}


==> arxiv/t3.tex <==
\begin{deluxetable*}{lcccccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablecaption{Spectral Line Indices \label{tab:lineindices}}
\tablehead{
  \colhead{Line} &
  \colhead{Line} &
  \colhead{Line} &
  \colhead{Cont. 1} &
  \colhead{Cont. 1} &
  \colhead{Cont. 2} &
  \colhead{Cont. 2} \\
  \colhead{Name} &
  \colhead{Center ($\mu$)} &
  \colhead{Width ($\mu$)} &
  \colhead{Center ($\mu$)} &
  \colhead{Width ($\mu$)} &
  \colhead{Center ($\mu$)} &
  \colhead{Width ($\mu$)} }
\startdata
Mg 1.50 & 1.504 &  0.004 &  1.498 &  0.0045 &  1.5095 &  0.0045 \\
K 1.52 & 1.5172 &  0.004 &  1.5105 &  0.004 &  1.523 &  0.004 \\
Mg 1.58 & 1.576 &  0.004 &  1.57 &  0.004 &  1.58 &  0.004 \\
Si 1.59 &  1.59 &  0.005 &  1.586 &  0.003 &  1.594 &  0.003 \\
CO 1.62 & 1.61975 &  0.0045 &  1.615 &  0.003 &  1.628 &  0.003 \\
CO 1.66 & 1.6625 &  0.004 &  1.6565 &  0.003 &  1.67 &  0.003 \\
Al 1.67 & 1.674 &  0.006 &  1.659 &  0.003 &  1.678 &  0.002 \\
1.70 dip & 1.7075 &  0.003 &  1.704 &  0.003 &  1.7145 &  0.003 \\
Mg 1.71 & 1.7115 &  0.003 &  1.704 &  0.003 &  1.7145 &  0.003 \\
Ca 1.98 & 1.982 & 0.013 & 1.9676 & 0.005 & 1.99775 & 0.005 \\
Na 2.21 & 2.2075 & 0.007 & 2.195 & 0.004 & 2.217 & 0.006 \\
Ca 2.26 & 2.264 & 0.007 & 2.258 & 0.0045 & 2.27 & 0.0045 \\
CO 2.3 & 2.30375 & 0.0225 & 2.288 & 0.007 & 2.3185 & 0.004 \\
CO 2.34 & 2.3455 & 0.003 & 2.3425 & 0.003 & 2.349 & 0.003 \\
\enddata
\end{deluxetable*}


==> arxiv/t4.tex <==
\begin{deluxetable}{lccc}
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablecaption{Water Indices \label{tab:waterindices}}
\tablehead{
  \colhead{Name} &
  \colhead{Band 1} &
  \colhead{Band 2} &
  \colhead{Band 3} }
\startdata
H$_2$O-H & 1.595-1.615 & 1.68-1.70 & 1.76-1.78 \\
H$_2$O-K & 2.18-2.20 & 2.27-2.29 & 2.36-2.38 \\
\enddata
\end{deluxetable}


==> arxiv/t5.tex <==
\begin{deluxetable*}{lcccccccccc}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Measured Spectral  Parameters  \label{tab:B59_spts}}
\tablehead{
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{low} &
  \colhead{} \\
  \colhead{Source} &
  \colhead{SpT}\tablenotemark{a} &
  \colhead{A$_H$} &
  \colhead{r$_J$} &
  \colhead{$\Delta$J-H} &
  \colhead{r$_H$} &
  \colhead{$\Delta$H-K} &
  \colhead{r$_K$} &
  \colhead{Br$\gamma$?} &
  \colhead{log $g$?} &
  \colhead{YSO} }
\startdata
\textrm{[BHB2007] 1} & K7  & 0.84 & 0.26 & 0.05 & 0.32 & 0.30 & 0.76 & Y & Y & Y \\
\textrm{[BHB2007] 2} & M3  & 0.68 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & W & Y & Y \\
\textrm{[BHB2007] 3} & M6  & 1.43 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & ? & N & ? \\
\textrm{[BHB2007] 4} & M5  & 0.74 & 0.26 & 0.10 & 0.39 & 0.16 & 0.62 & Y & Y & Y \\
\textrm{[BHB2007] 6} & M2  & 0.97 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & N & Y & Y \\
\textrm{[BHB2007] 7} & K5:  & 2.80 & 0.45 & 0.44 & 1.16 & 0.69 & 3.11 & Y & Y & Y \\ 
\textrm{[BHB2007] 8NW}\tablenotemark{b}& K/M: & 2.41 & \nodata & \nodata & 1.20 & 1.54 & 11.5 & N & ? & ? \\ 
\textrm{[BHB2007] 8SE}\tablenotemark{b}& M: & 4.54 & \nodata & \nodata & 0.26 & 3.89 & 1.34 & N & ? & ? \\ 
\textrm{[BHB2007] 9}  & K5  & 1.34 & 0.38 & 0.39 & 0.97 & 0.61 & 2.48 & Y & Y & Y \\
\textrm{[BHB2007] 12} & M5  & 3.00 & 0.26 & 0.13 & 0.42 & 0.27 & 0.73 & Y & Y & Y \\ 
\textrm{[BHB2007] 13NW}& M2 & 2.18 & 0.15 & 0.00 & 0.15 & 0.00 & 0.15 & W? & Y & Y \\
\textrm{[BHB2007] 14} &  K5 & 2.48 & 0.38 & 0.38 & 0.96 & 0.60 & 2.43 & Y & Y & Y \\ 
\textrm{[BHB2007] 15} &  M6 & 1.74 & 0.00 & 0.01 & 0.01 & 0.01 & 0.03 & N & Y & Y \\
\textrm{[BHB2007] 16} &  K4: & 1.83 & 0.32 & 0.09 & 0.44 & 0.12 & 0.61 & N & Y & Y \\
\textrm{[BHB2007] 18NE}& M5 & 0.60 & 0.26 & 0.15 & 0.45 & 0.25 & 0.83 & Y & Y & Y \\
\textrm{[BHB2007] 18SW}& M2: & 0.76 & 0.26 & 0.12 & 0.41 & 0.27 & 0.83 & W & Y & Y \\
\textrm{[BHB2007] 19} &  M3: & 1.36 & 0.25 & 0.0 & 0.25 & 0.00 & 0.25 & Y & Y? & Y \\
\textrm{[BHB2007] 20} &  M2 & 0.48 & 0.38 & 0.04 & 0.43 & 0.13 & 0.63 & Y & Y & Y \\
\textrm{[CLR2010] 2NE} &  M3 & 0.20 & 0.25 & 0.00 & 0.25 & 0.18 & 0.48 & W? & Y? & Y? \\
\textrm{[CLR2010] 2SW} &  M5 & 0.20 & 0.25 & 0.12 & 0.40 & 0.19 & 0.67 & Y & Y? & Y? \\
\textrm{[CLR2010] 1} &  M1 & 1.30 & 0.25 & 0.00 & 0.25 & 0.00 & 0.25 & N & Y & ? \\
\enddata
\tablenotetext{a}{Spectral types flagged with colons are derived from somewhat noisy spectra, resulting in less certain derived spectral types.}
\tablenotetext{b}{Spectra are extremely noisy, and lack data in the J band; measurements of r$_J$ and $\Delta$(J-H) are impossible, and other measurements are very low quality.}
\end{deluxetable*}


==> arxiv/t6.tex <==
\begin{deluxetable*}{lcccccccc}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Inferred Stellar Parameters  \label{tab:inferred_params}}
\tablehead{
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{} &
  \colhead{DM98 Age} &
\colhead{DM98 Mass} &
  \colhead{B98 Age} &
\colhead{B98 Mass} \\
  \colhead{Source} &
  \colhead{T$_{eff}$} &
  \colhead{BC$_H$} &
  \colhead{Log $\frac{L_{tot}}{L_{\odot}}$} &
  \colhead{Log $\frac{L_{stel}}{L_{\odot}}$} &
  \colhead{(Myr)} &
\colhead{(M$_{\odot}$)} &
  \colhead{(Myr)} &
\colhead{(M$_{\odot}$)}
}
\startdata
\textrm{[BHB2007] 1} & 4060. & 2.11 &  0.02 & -0.10 & 0.79 & 0.49 & 4.37 & 1.14 \\
\textrm{[BHB2007] 2} & 3346. & 2.37 & -0.03 & -0.03 & $\leq$0.07 & 0.20 & $\leq$1.0 & 0.60 \\
\textrm{[BHB2007] 3} & 2841. & 2.58 & -1.38 & -1.38 & 2.59  & 0.09 & $\leq$1.0 & 0.07 \\
\textrm{[BHB2007] 4} & 3009. & 2.51 & -0.75 & -0.89 & 1.04 & 0.14 & $\leq$1.0 & 0.14 \\
\textrm{[BHB2007] 6} & 3514. & 2.27 & -0.14 & -0.14 & 0.15 & 0.24 & $\leq$1.0 &  0.62 \\
\textrm{[BHB2007] 7} & 4350. & 2.02 &  0.12 &  -0.22 & 2.71 & 0.75  & 12.02 & 1.16 \\
\textrm{[BHB2007] 9} & 4350. & 2.02 & -0.37 & -0.67 & 23.4 & 0.79 & 50.11 & 0.77 \\
\textrm{[BHB2007] 12} & 3009. & 2.51 &  -1.12 & -1.27 & 2.77 & 0.14 & 1.38 & 0.1 \\
\textrm{[BHB2007] 13NW} & 3514. & 2.27 & 0.03 & -0.03 & 0.088 & 0.23 & $\leq$1.0 & 0.68 \\
\textrm{[BHB2007] 14} & 4350. & 2.02 & 0.05 & -0.24 & 3.03 & 0.77 & 12.59 & 1.13 \\
\textrm{[BHB2007] 15} & 2841. & 2.58 &  -0.90 & -0.91 & 0.28 & 0.11 & $\leq$1.0 & 0.12 \\
\textrm{[BHB2007] 16} & 4590. & 1.98 &   0.07  & -0.09 & 2.77 & 0.88 &  13.18 & 1.24 \\
\textrm{[BHB2007] 18NE} & 3009. & 2.51 &  -0.78 & -0.94 & 1.28 & 0.14 & $\leq$1.0 & 0.13 \\
\textrm{[BHB2007] 18SW} & 3514. & 2.27 &  -0.89 & -1.04 & 6.71 &  0.34 & 13.2 & 0.46  \\
\textrm{[BHB2007] 19} & 3346. & 2.37 &  -1.37 & -1.47 & 16.6 &  0.26 &  19.1 & 0.27 \\ 
\textrm{[BHB2007] 20} & 3514. & 2.27 &  -0.44 & -0.60 &  1.37 &  0.30 &    3.47 & 0.50 \\
\textrm{V359 Oph} & 4060. & 2.11 & -0.36 & -0.36 & 2.42 & 0.61 & 10.47 & 1.02 \\
\textrm{Lk H$\alpha$ 345} & 4060. & 2.11 & -0.19 & -0.39 & 2.83 & 0.63 & 10.96 & 1.00 \\
\tableline
\textrm{[CLR2010] 2NE} & 3346. & 2.37 & -0.59 & -0.72 & 1.28 & 0.22 &   2.19 & 0.33 \\
\textrm{[CLR2010] 2SW} & 3009. & 2.51 & -0.70 & -0.84 & 0.54 & 0.13 &  $\leq$1.0  &  0.14 
\enddata
\end{deluxetable*}

